CreDes: Causal Reasoning Enhancement and Dual-End Searching for Solving Long-Range Reasoning Problems using LLMs

Large language models (LLMs) have demonstrated limitations in handling combinatorial optimization problems involving long-range reasoning, partially due to causal hallucinations and huge search space. As for causal hallucinations, i.e., the inconsistency between reasoning and corresponding state transition, this paper introduces the Causal Relationship Enhancement (CRE) mechanism combining cause-effect interventions and the Individual Treatment Effect (ITE) to guarantee the solid causal rightness between each step of reasoning and state transition. As for the long causal range and huge search space limiting the performances of existing models featuring single-direction search, a Dual-End Searching (DES) approach is proposed to seek solutions by simultaneously starting from both the initial and goal states on the causal probability tree. By integrating CRE and DES (CreDes), our model has realized simultaneous multi-step reasoning, circumventing the inefficiencies from cascading multiple one-step reasoning like the Chain-of-Thought (CoT). Experiments demonstrate that CreDes significantly outperforms existing State-Of-The-Art (SOTA) solutions in long-range reasoning tasks in terms of both accuracy and time efficiency.

==> figures/overview.tex <==
\begin{tikzpicture}
\definecolor[grey]{grey}{RGB}{120, 120, 120}
\definecolor{midgrey}{RGB}{200, 200, 200}
\definecolor[lightgrey]{lightgrey}{RGB}{220, 220, 220}
\definecolor{redcolor}{RGB}{205, 92, 92}
\definecolor{greencolor}{RGB}{100,170,110} %
\definecolor{datacolor}{RGB}{60,60,60} %
\definecolor{refmodelcolor}{RGB}{222, 143, 5} 
\tikzstyle{my_step} = [text=gray, font=\itshape\LARGE, align=center, text width=6cm]
\tikzstyle{box} = [rectangle, rounded corners, fill=lightgray!50, text centered, text width=6cm, font=\large, minimum height=2.5cm, font=\LARGE]
\tikzstyle{arrow} = [->, thick, >=stealth, line width=1mm, color=grey]
\tikzstyle{dashedline} = [draw=lightgray, thick, dash pattern=on 0pt off 3pt on 5pt off 3pt, line width=0.5mm]

\tikzstyle{dataNode} = [
      rectangle, 
      text=white, 
      fill=lightgrey, 
      minimum height=5.4cm, 
      minimum width=8cm, 
      align=center, 
      rounded corners
  ]

  \tikzstyle{featuresNode} = [
      rectangle, 
      text=white, 
      fill=lightgrey, 
      minimum height=1.6cm, 
      minimum width=8cm, 
      align=center, 
      rounded corners
  ]

  \tikzstyle{featureNode} = [
    rectangle,
    fill=redcolor,
    minimum height=1.2cm, %
    minimum width=3.6cm,  %
    rounded corners,
    inner sep=1mm,
    anchor=west,
    font=\large
  ]

  \tikzstyle{approachNode} = [
      rectangle, 
      text=white, 
      fill=lightgrey, 
      minimum height=8cm, 
      minimum width=8cm, 
      align=center, 
      rounded corners
  ]
  \tikzstyle{smallDataNode} = [
    rectangle,
    fill=greencolor,
    minimum height=4.68cm, %
    minimum width=5.4cm,  %
    rounded corners,
    inner sep=0,
    anchor=west,
  ]

  \tikzstyle{smallCategoryNode} = [
    rectangle,
    fill=greencolor,
    minimum height=1.48cm, %
    minimum width=1.48cm,  %
    rounded corners,
    inner sep=0,
    anchor=west,
  ]

  \tikzstyle{textNode} = [
    rectangle,
    minimum height=2cm, %
    minimum width=2.4cm,  %
    inner sep=0,
    font=\Large
  ]

  \tikzstyle{titleNode} = [
    rectangle,
    inner sep=0,
    font=\LARGE,
    color=grey
  ]

  \tikzstyle{imagenode} = [
    rectangle,
    minimum height=0.8cm, %
    minimum width=0.8cm,  %
    inner sep=0,
  ]

  \tikzstyle{modelNode} = [
    rectangle,
    fill=greencolor,
    minimum height=0.7cm, %
    minimum width=3.6cm,  %
    rounded corners,
    inner sep=0,
    anchor=west,
    font=\Large
  ]

  \tikzstyle{categoryNode} = [
    rectangle,
    fill=greencolor,
    minimum height=1.3cm, %
    minimum width=1.3cm,  %
    rounded corners,
    inner sep=0,
    anchor=west,
  ]

  \tikzstyle{vector} = [
    rectangle,
    minimum height=3cm, %
    minimum width=1cm,  %
    inner sep=0,
    font=\fontsize{22}{34}\selectfont
  ]

  \tikzstyle{mle} = [
    rectangle,
    fill=lightgrey,
    inner sep=1mm,
    font=\Large
  ]

  \tikzstyle{everythingNode} = [
      rectangle, 
      fill=midgrey, 
      minimum height=3.2cm, 
      minimum width=7.4cm, 
      align=center, 
      rounded corners
  ]

  

  \node[dataNode] (data) at (0, 0) {};

  \node[titleNode, anchor=south, yshift=2mm] (title) at (data.north) {
    \textit{Preference Datasets}
  };

  \node[smallDataNode, anchor=north west, xshift=4mm, yshift=-4mm] (data1) at (data.north west) {
  };

  \node[imagenode, anchor=north, yshift=-0mm] (image1) at (data1.north) {
    \includegraphics[width=1.2cm]{figures/overview/code.png}
  };

  \node[textNode, anchor=north] (TextData1) at (image1.south) {

    \begin{tabular}{@{}c@{}}
      $\left\langle Q_1, m^{(0)}_1, m^{(1)}_1,  J_1, r_1 \right\rangle$ \\
      \vspace{-2mm}
      $\left\langle Q_2, m^{(0)}_2, m^{(1)}_2, J_2, r_2\right\rangle$ \\
      $\vdots$ \\
      $\left\langle Q_{n}, m^{(0)}_{n}, m^{(1)}_{n}, J_{n}, r_{n} \right\rangle$
  \end{tabular}
  };

  \node[smallCategoryNode, anchor=north west, xshift=4mm] (data2) at (data1.north east) {};

  \node[imagenode, anchor=north, yshift=-1mm] (image2) at (data2.north) {
    \begin{tabular}{c}
    \vspace{-1mm}
    \includegraphics[width=0.9cm]{figures/overview/dragon.png} \\
    $\langle\dots\rangle$ \\
    \end{tabular}
    
  };

  \node[smallCategoryNode, yshift=-1mm, anchor=north] (data3) at (data2.south) {};

  \node[imagenode, anchor=north, yshift=-1mm] (image3) at (data3.north) {
    \begin{tabular}{c}
      \vspace{-2mm}
      \includegraphics[width=1cm]{figures/overview/calculator.png} \\
      $\langle\dots\rangle$ \\
      \end{tabular}
  };

  \node[smallCategoryNode, yshift=-1mm, anchor=north] (data4) at (data3.south) {};

  \node[imagenode, anchor=north, yshift=-1mm] (image4) at (data4.north) {
    \begin{tabular}{c}
      \vspace{-2mm}
      \includegraphics[width=1.0cm]{figures/overview/bot.png} \\
      $\langle\dots\rangle$ \\
      \end{tabular}
  };

  \node[featuresNode, anchor=north, yshift=-9mm] (features) at (data.south) {};

  \node[titleNode, anchor=south, yshift=2mm] (title) at (features.north){
    \textit{Continuous Features}
  };

  \node[featureNode, anchor=north west, xshift=2mm, yshift=-2mm] (feature1) at (features.north west) {
      \includegraphics[width=1.2cm]{figures/overview/length.png}
  };

  \node[featureNode, anchor=west, xshift=3mm] (feature2) at (feature1.east) {
      \includegraphics[width=1.2cm]{figures/overview/guideline.png}
  };

  \node[approachNode, anchor=north east, xshift=-1cm] (traditional) at (data.north west) {};

  \draw[arrow] (data.west) -- (traditional.east |- data.west);

  \node[titleNode, anchor=south, yshift=2mm] (titleTraditional) at (traditional.north) {
    \textit{Standard Approach}
  };

  \node[categoryNode, anchor=north west, yshift=-2mm, xshift=18mm] (category1) at (traditional.north west) {\includegraphics[width=1.1cm]{figures/overview/code.png}};

  \node[vector, anchor=north, yshift=-14mm] (vector1) at (category1.south) {
    \begin{tabular}{c}
      $R^1_{\includegraphics[width=0.5cm]{figures/overview/code.png}}$ \\
      $R^2_{\includegraphics[width=0.5cm]{figures/overview/code.png}}$ \\
      $\vdots$ \\
      $R^k_{\includegraphics[width=0.5cm]{figures/overview/code.png}}$
  \end{tabular}
  };

  \draw[arrow] (category1.south) -- (vector1.north) node[midway, mle] {MLE};


  \node[categoryNode, anchor=west, xshift=2.5mm] (category2) at (category1.east) {\includegraphics[width=1.1cm]{figures/overview/dragon.png}};

  \node[vector, anchor=north, yshift=-14mm] (vector2) at (category2.south) {
    \begin{tabular}{c}
      $R^1_{\includegraphics[width=0.5cm]{figures/overview/dragon.png}}$ \\
      $R^2_{\includegraphics[width=0.5cm]{figures/overview/dragon.png}}$ \\
      $\vdots$ \\
      $R^k_{\includegraphics[width=0.5cm]{figures/overview/dragon.png}}$
  \end{tabular}
  };

  \draw[arrow] (category2.south) -- (vector2.north) node[midway, mle] {MLE};

  \node[categoryNode, anchor=west, xshift=2.5mm] (category3) at (category2.east) {\includegraphics[width=1.1cm]{figures/overview/calculator.png}};

  \node[vector, anchor=north, yshift=-14mm] (vector3) at (category3.south) {
    \begin{tabular}{c}
      $R^1_{\includegraphics[width=0.5cm]{figures/overview/calculator.png}}$ \\
      $R^2_{\includegraphics[width=0.5cm]{figures/overview/calculator.png}}$ \\
      $\vdots$ \\
      $R^k_{\includegraphics[width=0.5cm]{figures/overview/calculator.png}}$
  \end{tabular}
  };

  \draw[arrow] (category3.south) -- (vector3.north) node[midway, mle] {MLE};

  \node[categoryNode, anchor=west, xshift=2.5mm] (category4) at (category3.east) {\includegraphics[width=1.1cm]{figures/overview/bot.png}};


  \node[vector, anchor=north, yshift=-14mm] (vector4) at (category4.south) {
    \begin{tabular}{c}
      $R^1_{\includegraphics[width=0.5cm]{figures/overview/bot.png}}$ \\
      $R^2_{\includegraphics[width=0.5cm]{figures/overview/bot.png}}$ \\
      $\vdots$ \\
      $R^k_{\includegraphics[width=0.5cm]{figures/overview/bot.png}}$
  \end{tabular}
  };

  \draw[arrow] (category4.south) -- (vector4.north) node[midway, mle] {MLE};

  \node[vector, anchor=east, xshift=2mm] (vectorModels) at (vector1.west) {
    \begin{tabular}{c}
      $m_1 \hspace{-1.5mm}\rightarrow\hspace{-1.5mm}$ \\
      $m_2 \hspace{-1.5mm}\rightarrow\hspace{-1.5mm}$ \\
      $\vdots$ \\
      $m_k\hspace{-1.5mm}\rightarrow\hspace{-1.5mm}$
  \end{tabular}
  };


  \node[approachNode, anchor=north west, xshift=1cm] (polyrating) at (data.north east) {};

  \draw[arrow] (data.east) -- (polyrating.west |- data.east);
  \draw[arrow] (features.east) -- (polyrating.west |- features.east);

  \node[titleNode, anchor=south, yshift=4mm] (titlePolyrating) at (polyrating.north) {
    \tool
  };

  \node[everythingNode, anchor=north, yshift=-4mm] (everything) at (polyrating.north) {};

  \node[categoryNode, anchor=north west, yshift=-2mm, xshift=5mm] (category1Poly) at (everything.north west) {\includegraphics[width=1.1cm]{figures/overview/code.png}};

  \node[categoryNode, anchor=west, xshift=4mm] (category2Poly) at (category1Poly.east) {\includegraphics[width=1.1cm]{figures/overview/dragon.png}};

  \node[categoryNode, anchor=west, xshift=4mm] (category3Poly) at (category2Poly.east) {\includegraphics[width=1.1cm]{figures/overview/calculator.png}};

  \node[categoryNode, anchor=west, xshift=4mm] (category4Poly) at (category3Poly.east) {\includegraphics[width=1.1cm]{figures/overview/bot.png}};

  \node[featureNode, anchor=north west, xshift=5mm, yshift=-18mm, minimum width=3.02cm] (feature1Poly) at (everything.north west) {
      \includegraphics[width=1.2cm]{figures/overview/length.png}
  };

  \node[featureNode, anchor=west, xshift=4mm, minimum width=3.02cm] (feature2Poly) at (feature1Poly.east) {
      \includegraphics[width=1.2cm]{figures/overview/guideline.png}
  };


  \node[everythingNode, anchor=north west, yshift=-20mm, minimum width=5.3cm, minimum height = 2cm, font=\LARGE] (models) at (everything.south west) {
    $R_{\text{task}}^m = R^m_\text{base} + \beta_{\text{task}}^m$
  };

  \node[titleNode, anchor=south, yshift=2mm] (titleModels) at (models.north) {
    \textit{Model-Specific}
  };

  \node[everythingNode, anchor=north east, yshift=-20mm, minimum width=1.8cm, minimum height = 2cm, font=\LARGE] (shared) at (everything.south east) {
    \begin{tabular}{c}
      $\alpha_{{\includegraphics[width=0.5cm]{figures/overview/length.png}}}$ \\
      $\alpha_{{\includegraphics[width=0.5cm]{figures/overview/guideline.png}}}$
    \end{tabular}
  };

  \node[titleNode, anchor=south, yshift=2mm] (titleShared) at (shared.north) {
    \phantom{p}\textit{Shared}\phantom{p}
  };
  \draw[arrow] (everything.south) -- (everything.south |- titleModels.north) node[midway, mle] {MAP};



\end{tikzpicture}

==> paper_files/abstract.tex <==
\begin{abstract}
    Rating-based human evaluation has become an essential tool to accurately evaluate the impressive performance of Large language models (LLMs). However, current rating systems suffer from several critical limitations. Specifically, they fail to account for human biases that significantly influence evaluation results, require large and expensive preference datasets to obtain accurate ratings, and do not facilitate meaningful comparisons of model ratings across different tasks. To address these issues, we introduce \tool, an expressive and flexible rating system based on maximum a posteriori estimation that enables a more nuanced and thorough analysis of model performance at lower costs. \tool can detect and quantify biases affecting human preferences, ensuring fairer model comparisons. Furthermore, \tool can reduce the cost of human evaluations by up to $41\%$ for new models and up to $77\%$ for new tasks by leveraging existing benchmark scores. Lastly, \tool enables direct comparisons of ratings across different tasks, providing a comprehensive understanding of an LLMs' strengths, weaknesses, and relative performance across different applications.\footnote{Code available at \url{https://github.com/JasperDekoninck/Polyrating}.}
    

    
\end{abstract}

==> paper_files/acknowledgements.tex <==
\section*{Acknowledgements}
This work was funded in part by the Swiss National Science Foundation (SNSF) [200021\_207967].

This work has been done as part of the EU grant ELSA (European Lighthouse on Secure and Safe AI, grant agreement no. 101070617). Views and opinions expressed are however those of the authors only and do not necessarily reflect those of the European Union or European Commission. Neither the European Union nor the European Commission can be held responsible for them.

The work has received funding from the Swiss State Secretariat for Education, Research and Innovation (SERI).

==> paper_files/background.tex <==
\section{Rating Systems}\label{sec:background}

In this section, we introduce the necessary notation to formalize rating systems for LLMs. 

\paragraph{Preference Datasets} A rating system requires the availability of a preference dataset, which consists of $n$ games that capture the preferences of a judge. In language model evaluation, a game $g$ consists of a user query $Q$, two language models $m_0$ and $m_1$, and a judge $J$. The result $r$ of the game is determined by the judge's preference for one of the completions and is $1$ if $m_1$ beats $m_0$, denoted as $m_1 \succ m_0$, and $0$ if $m_0 \succ m_1$. Thus, we can represent a game $g$ as a tuple $\langle Q, m_0, m_1, J, r \rangle$.


\paragraph{Rating System} For a given set of $k$ models, a rating system assigns a score $\gamma_i \in \mathbb{R}^+$ to model $m_i$, indicating the relative skill of the model on the task. With these scores, the probability that $m_i$ wins against $m_j$ can be computed using the Bradley-Terry model (BT-model) \citep{bradley1952rank}:
\begin{equation*}\label{eq:bradley-terry}
P(m_i \succ m_j | \gamma_i, \gamma_j) = \frac{\gamma_i}{\gamma_i + \gamma_j}.
\end{equation*}
In most rating systems the scores are parametrized using the exponential function $\gamma_i = \exp(R_i / 400)$ where $R_i$ the rating of $m_i$ and $400$ is a constant used to scale the ratings \citep{elo2008rating, glicko}. 


\paragraph{Rating Optimization} To determine the ratings of the models, a rating system aims to maximize predictive capabilities for the observed outcomes of the games. The maximum likelihood estimate for these observed outcomes in the BT-model can be found by minimizing the logistic loss

\begin{equation}\label{eq:logistic-loss}
    \mathcal{L}(D, \mathbf{R}) = -\sum_{g \in D} \Big(g_{\text{r}} \log P(g_{m_1} \succ g_{m_0} | \mathbf{R}) + (1 - g_{\text{r}}) \log P(g_{m_0} \succ g_{m_1} | \mathbf{R}) \Big)
\end{equation}
for a dataset of games $D = (g_1, \dots, g_n)$ and ratings $\mathbf{R} = (R_1, \dots, R_k)$. Thus, the optimal ratings can be obtained by computing $\argmin_{\mathbf{R}} \mathcal{L}(D, \mathbf{R})$. To obtain ratings for specific tasks, the optimization is performed separately for each task on the task-specific dataset $D$.

\paragraph{Incorporating Draws} However, the BT-model ignores the possibility of draws in games. Following the approach by the Chatbot Arena \citep{chatbot_arena}, we can generalize the BT-model by setting the outcome $g_{r}$ equal to $0.5$ for draws to obtain model ratings that can incorporate these draws. Although we explore several alternatives to the BT-model that more explicitly model draws in \cref{app:alternatives}, we found they did not offer significant advantages in practice.

==> paper_files/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

We introduced \tool, a multivariate rating system specifically designed for language model evaluation. \tool enables a more comprehensive evaluation of LLMs by capturing biases and dependencies on both continuous and categorical features in the evaluation. We demonstrated the existence and influence of several biases, such as length and position bias, and compared these biases between human and LLM-based judges. Furthermore, we showed that \tool can leverage existing data to increase sample efficiency by $41\%$ and reduce the costs of human evaluations for new tasks by up to $77\%$. Finally, we showed that \tool can provide a more reliable performance comparison of the same language model across different tasks by solving the shift-invariance of the ratings across multiple dimensions.

==> paper_files/experiments.tex <==
\section{Evaluation}\label{sec:experiments}

We perform a series of experiments with \tool that showcase its ability to quantify the influence of biases on the ratings of the models (\cref{sec:experiments:bias}), its improved sample efficiency for various use-cases (\cref{sec:experiments:convergence}), and its ability to obtain reliable and comparable multivariate leaderboards (\cref{sec:experiments:leaderboards}).

\subsection{Bias Detection}\label{sec:experiments:bias}



We use \tool to quantify the influence of biases in both human and LLM-based evaluation using a public subset of the Chatbot Arena \citep{kaggle-lmsys} and Wildbench \citep{lin2024wildbench}. This enables an accurate estimation of the effects of these biases on model ratings and allows us to compare the influence of these biases between human and LLM-based judges.

\paragraph{Biases} We briefly explain the measured biases and refer to \cref{app:details} for a full overview of all biases along with their functional form. We include the well-known length bias \citep{alpacelengthcontrolled,singhal2023long}, which measures bias with respect to the length of the completion, and position bias \citep{shi2024judging,wang2023large}, which measures bias with respect to the order of the models in the game. We further use classifiers \citep{formality,sentiment} to evaluate the influence of formality and sentiment of the model's output. Finally, we compute the repetitiveness of the answer by measuring the number of unique tokens in the completion and check the influence of the readability of an answer using the Flesch Reading Ease score \citep{kincaid1975derivation}. We model all of these biases as shared features when fitting \tool, allowing us to accurately estimate their influence on the resulting ratings.

\begin{table}[t]
    \centering
    \footnotesize
    \caption{Fitted coefficients for the biases and their average influence on model ratings for both human and LLM-based evaluation. The functional form of $f_{\text{bias}}$ used for each bias can be found in \cref{app:details}. The influence is computed as $\mathbb{E}_g(\alpha_{\text{bias}} \cdot |f_{\text{bias}}(g, 0) - f_{\text{bias}}(g, 1)|)$.}
    \label{tab:biases}
    \begin{subtable}[t]{0.48\textwidth}
        \centering
        \caption{Human Evaluation}
        \label{tab:biases:human}
        \begin{tabular}{lcc}
            \toprule
            Bias & {Coefficient $(\alpha)$} & {Influence $(\mathbb{E})$} \\
            \midrule
            Length & $\phantom{-}130.74_{\pm 7.3\phantom{0}}$ & $\phantom{-}40.84_{\pm 2.3}$ \\
            Position & $\phantom{-00}2.70_{\pm 2.4\phantom{0}}$ & $\phantom{-0}2.70_{\pm 2.4}$ \\
            Formality & $-119.89_{\pm 11.3}$ & $-15.17_{\pm 1.4}$ \\
            Sentiment & $\phantom{-0}57.42_{\pm 11.1}$ & $\phantom{-0}7.90_{\pm 1.5}$ \\
            Repetitiveness & $- \phantom{0} 22.10_{\pm 8.6\phantom{0}}$ & $-\phantom{0}4.64_{\pm 1.8}$ \\
            Readability & $\phantom{-0}72.93_{\pm 11.9}$ & $\phantom{-}10.75_{\pm 1.8}$ \\
            \bottomrule
        \end{tabular}
        
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.48\textwidth}
        \centering
        \caption{LLM-based Evaluation}
        \label{tab:biases:llm}
        \begin{tabular}{lcc}
            \toprule
            Bias & {Coefficient $(\alpha)$} & {Influence $(\mathbb{E})$} \\
            \midrule
            Length & $\phantom{-}251.87_{\pm 7.2}$ & $\phantom{-}48.48_{\pm 1.4}$ \\
            Position & $\phantom{-0}37.53_{\pm 1.1}$ & $\phantom{-}37.53_{\pm 1.1}$ \\
            Formality & $-\phantom{0}37.56_{\pm 6.9}$ & $-\phantom{0}4.31_{\pm 0.8}$ \\
            Sentiment & $\phantom{-00}4.31_{\pm 6.5}$ & $\phantom{-0}0.43_{\pm 0.7}$ \\
            Repetitiveness &  $\phantom{-0}75.04_{\pm 8.3}$ & $\phantom{-0}9.12_{\pm 1.0}$ \\
            Readability & $-\phantom{0}32.56_{\pm 8.0}$ & $-\phantom{0}3.92_{\pm 1.0}$ \\
            \bottomrule
        \end{tabular}
        
    \end{subtable}
    \vspace{-2mm}
\end{table}

\paragraph{Results} \cref{tab:biases} shows the effects of these biases on both human and LLM-based judges. We present both the coefficient $\alpha_{\text{bias}}$ and the average influence this coefficient has on model ratings for given queries, i.e. $\mathbb{E}_g(\alpha_{\text{bias}} \cdot |f_{\text{bias}}(g, 0) - f_{\text{bias}}(g, 1)|)$. To put these numbers into context, the difference between the first and the tenth best models in the Chatbot Arena is $50$ rating points.

\paragraph{Discussion for Length and Position Bias} We recover prior results on length and position bias for both human and LLM-based judges \citep{alpacelengthcontrolled,singhal2023long,shi2024judging,wang2023large}. Length bias is significant in both paradigms, though more so for LLM-based judges. This explains why length-controlling techniques achieve higher correlation with human judges \citep{alpacelengthcontrolled}. In contrast, position bias is only significant for LLM-based judges. Furthermore, in contrast to prior work, we can now estimate the effects of these biases on the ratings of the models, with position bias gaining a model around $38$ rating points when using an LLM-based judge and length bias gaining $41$ and $48$ rating points for human and LLM-based judges respectively. 

\paragraph{Discussion for Other Biases} The other biases reveal interesting patterns. First, all biases differ significantly between human and LLM-based judges. For instance, while readability increases the rating of a model by $11$ points for human judges, it decreases the rating by $4$ points for LLM-based judges. This indicates that LLM-based judges prefer denser text, while human judges prefer more readable text. Furthermore, we find that sentiment and formality have a significant influence on human judges, gaining models $8$ and $15$ rating points respectively. In contrast, LLM-based judges are indifferent to sentiment and not influenced as much by formality. Lastly, we find that repetitiveness decreases rating on average by $4$ rating points for human judges, while for LLM-based judges, it increases the rating by $9$ points.

\subsection{Improved Sample Efficiency}\label{sec:experiments:convergence}

We demonstrate that \tool is more sample-efficient compared to traditional univariate approaches and therefore reduces the cost of human evaluation.

\paragraph{Dataset} We use the full Chatbot Arena dataset \citep{chatbot_arena}, which contains over one million questions across various tasks. Each question is answered by two models and judged by the human that posed the question. We use the tasks that contain Chinese, code-based, and hard questions for this experiment and refer for a full description of these tasks to \cref{app:details}.


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/is_chinese_comparison.pdf}
        \vspace{-6mm}
        \caption{Chinese questions}
        \label{fig:single-cat:chinese}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/is_code_comparison.pdf}
        \vspace{-6mm}
        \caption{Code-based questions}
        \label{fig:single-cat:code}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/is_hard_comparison.pdf}
        \vspace{-6mm}
        \caption{Hard questions}
        \label{fig:single-cat:hard}
    \end{subfigure}
    \vspace{-2mm}
    \caption{Comparison between \tool and univariate baseline for different tasks. The $x$-axis shows the number of samples of the task the rating systems are using. The logistic loss shown is normalized by subtracting the loss of the best possible rating for that task. The grey horizontal line indicates the loss of a rating system that assigns the same rating to all models.}
    \label{fig:single-cat}
\end{figure}


\paragraph{New Task} We first showcase the improved sample efficiency when obtaining ratings for a new task. For this purpose, we vary the number of available questions from the task and compute the logistic loss with respect to a hidden test set. In this process, and in all further experiments of this subsection, \tool is allowed to use all questions in the dataset that do not belong to the task. Thus, we model the rating of a model $m$ for a game $g$ as $R^{m}_\text{base} + \beta^{m}_{\text{task}} \cdot \iverson{g \in D_{\text{task}}}$ where $D_{\text{task}}$ is the dataset of all games from the task. The standard deviation of the prior on $\beta^{m}_{\text{task}}$ is determined by running cross-validation on the current training set. 

Results for the three tasks are shown in \cref{fig:single-cat}. We find that \tool converges much faster than the univariate baseline. Specifically, the increase in sample efficiency when collecting $10000$ samples is $58\%$, $38\%$, and $77\%$ for respectively the Chinese, code-based, and hard questions. Thus, \tool can cut the cost of obtaining ratings for new tasks by up to fourfold.


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/wildbench_comparison.pdf}
        \vspace{-6mm}
        \caption{LLM-based evaluation}
        \label{fig:llm-convergence}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mixeval_comparison.pdf}
        \vspace{-6mm}
        \caption{Traditional benchmark}
        \label{fig:classical-convergence}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/is_chinese_is_code_comparison.pdf}
        \vspace{-6mm}
        \caption{Decomposable task}
        \label{fig:multi-cat}
    \end{subfigure}
    \vspace{-2mm}
    \caption{Comparison between \tool and the univariate baseline when leveraging information from existing benchmarks. For the left and middle plot, the $x$-axis shows the number of human annotations used. For the right plot, the $x$-axis shows the amount of samples from the Chinese code task. The logistic loss is normalized by subtracting the loss of the best possible rating. The grey horizontal line indicates the loss of a rating system that assigns the same rating to all models.}
    \vspace{-1mm}
    \label{fig:other-convergences}
\end{figure}

\paragraph{LLM-based Judge Improves Sample Efficiency} LLM-based preferences are much cheaper to obtain than human preferences. Therefore, LLM-based judges are often used to obtain model ratings, despite being less reliable than human judges. However, \tool can further leverage these ratings to converge faster to the ratings corresponding to human judges. Specifically, we model the rating of a model $m$ for a game $g$ as 
\begin{equation*}
    R^m(g) = R^m_{\text{base}} + \alpha_{1} \cdot \iverson{g \in D_\text{LLM}} \cdot \log(\text{length}(g_{y_m})) + \beta^m_{1} \cdot \iverson{g \in D_\text{LLM}}
\end{equation*}
where $\text{length}(g_{y_m})$ is the length of the models' completion for the given question. We use the public dataset from Wildbench \citep{lin2024wildbench} to obtain our LLM-based evaluation. \cref{fig:llm-convergence} shows the logistic loss on a test set of the Chatbot Arena for a varying amount of human annotations. We find that \tool converges faster to the optimal ratings than the univariate baseline. Specifically, the increase in sample efficiency when collecting $10000$ human annotations is $38\%$.

\paragraph{Classical Benchmarks Improve Sample Efficiency} Obtaining results from classical benchmarks is even cheaper than LLM-based evaluations. We leverage these benchmarks to increase sample efficiency. To do so, we first convert a benchmark to a preference dataset based on model accuracy as explained in \cref{sec:tool}. We then model rating as $R^m_{\text{base}} + \beta^m_{1} \cdot \iverson{g \in D_\text{benchmark}}$ and apply \tool to increase sample efficiency for human evaluation. We specifically use the MixEval-Hard \citep{mixeval} benchmark and show results in \cref{fig:classical-convergence}. We find that \tool significantly increases the sample efficiency. Specifically, when collecting $10000$ samples efficiency increases by $41\%$. 

\paragraph{Decomposable Task} Some tasks can be decomposed into two or more subtasks. If these subtasks are prevalent in the dataset, but their combination is not, \tool can obtain more reliable ratings for the combined task. For example, Chinese code-based questions are rare  in the Chatbot Arena, but both Chinese questions and code-based questions are prevalent. For this example, we can model the rating of a model $m$ for a game $g$ as 
\begin{equation*}
    R^m(g) = R^m_{\text{base}} + \beta^m_{1} \cdot \iverson{g \in D_\text{chinese}} + \beta^m_{2} \cdot \iverson{g \in D_\text{code}} + \beta^m_{3} \cdot \iverson{g \in D_\text{code} \cap D_\text{chinese}}.
\end{equation*}
\cref{fig:multi-cat} shows the logistic loss for varying numbers of Chinese code-based questions from the Chatbot Arena. \tool's logistic loss at the start is almost as low as the univariate baseline's at the end, with a sample efficiency improvement of $25\%$ when obtaining $10000$ samples.




\subsection{Multivariate Leaderboard}\label{sec:experiments:leaderboards}

We now compare separately fitted univariate leaderboards with a multivariate leaderboard fitted using \tool. Since the univariate approach is shift-invariant, we need to fix the shifting constant for each task. We follow the approach of the Chatbot Arena and set the constant by fixing the rating of Mixtral-8x7b-Instruct-v0.1 to $1114$ for all tasks. We will show that this approach fails to provide comparable ratings for the models in the leaderboard.


\paragraph{Results} \cref{tab:leaderboard-small} and \cref{tab:leaderboard-small-single} show the ratings of several models in the leaderboard fitted using \tool and a univariate approach respectively. For a full overview of all models, we refer to \cref{app:results}. By examining the modifiers computed by \tool, we immediately see the downside of the univariate approach. In both the English and Chinese tasks, the Mixtral model performs very differently compared to the other tasks. Fixing the shifting constant using this model results in significant ratings shifts for these two tasks compared to the base rating. 

This effect is most apparent in the Chinese task. Almost all models gain substantial ratings in the univariate approach, even though yi-large-preview is the only model built bilingually from the ground up. In contrast, \tool shows that yi-large-preview is the only model that gains rating in this task. Similarly, llama-3-70b-instruct, a model specifically trained for English, gains only 22 rating points in the English task using the univariate approach, whereas \tool shows it gains 67 rating points, aligning more with expectations. The last two tasks show more similarities between the two approaches, but we note that the arbitrary shifting constant for each task makes it very hard to actually trust these modifiers in the univariate approach.

\begin{table}[t]
    \caption{Several models in a multidimensional leaderboard fitted using \tool. The given rank of the models indicates its rank in the complete leaderboard shown in \cref{tab:leaderboard} in \cref{app:results}.}
    \vspace{-2mm}
    \label{tab:leaderboard-small}
    \centering
    \footnotesize
    \begin{tabular}{lllllll}
    \toprule
    Rank & Model Name & Rating & English & Chinese & Hardness & Code \\
    \midrule
    1 & gpt-4o-2024-05-13 & $1297_{\pm 4.4} $ & $-13_{\pm 7.4} $ & $-\phantom{00}3_{\pm 8.7} $ & $\phantom{-} 13_{\pm 7.5} $ & $\phantom{-} 15_{\pm 8.0} $ \\
    2 & claude-3-5-sonnet-20240620 & $1286_{\pm 7.1} $ & $-29_{\pm 10.7} $ & $-\phantom{0}19_{\pm 13.8} $ & $\phantom{-} 14_{\pm 11.0} $ & $\phantom{-} 44_{\pm 12.6} $ \\
    12 & yi-large-preview & $1237_{\pm 4.3} $ & $-\phantom{0}4_{\pm 7.6} $ & $\phantom{-} \phantom{0}37_{\pm 8.5} $ & $\phantom{-} 17_{\pm 7.6} $ & $\phantom{-} 11_{\pm 8.3} $ \\
    26 & llama-3-70b-instruct & $1187_{\pm 2.9} $ & $\phantom{-} 67_{\pm 6.0} $ & $-\phantom{0}51_{\pm 5.4} $ & $-\phantom{0}1_{\pm 5.6} $ & $-10_{\pm 6.1} $ \\
    56 & mixtral-8x7b-instruct-v0.1 & $1114_{\pm 4.1} $ & $\phantom{-} 25_{\pm 7.1} $ & $-\phantom{0}37_{\pm 7.3} $ & $\phantom{-} 10_{\pm 6.8} $ & $-\phantom{0}4_{\pm 7.6} $ \\
    \bottomrule
    \end{tabular}

\end{table}

\begin{table}[t]
    \caption{Several models in the leaderboard fitted using a unidimensional approach where each task is fitted separately. Modifiers for the tasks are shown instead of the fitted rating to make comparison with \tool easier. The complete leaderboard is shown in \cref{tab:leaderboard-single} in \cref{app:results}.}
    \label{tab:leaderboard-small-single}
    \centering
    \footnotesize
    \begin{tabular}{lllllll}
    \toprule
    Rank & Model Name & Rating & English & Chinese & Hardness & Code \\
    \midrule
    1 & gpt-4o-2024-05-13 & $1283_{\pm 3.2} $ & $-19_{\pm 5.2} $ & $\phantom{-} \phantom{0}52_{\pm 10.4} $ & $\phantom{-} \phantom{0}5_{\pm 6.7} $ & $\phantom{-} 13_{\pm 7.8} $ \\
    2 & claude-3-5-sonnet-20240620 & $1267_{\pm 4.8} $ & $-23_{\pm 8.1} $ & $\phantom{-} \phantom{0}45_{\pm 14.4} $ & $\phantom{-} 11_{\pm 10.1} $ & $\phantom{-} 35_{\pm 11.3} $ \\
    10 & yi-large-preview & $1233_{\pm 3.3} $ & $-19_{\pm 5.6} $ & $\phantom{-} \phantom{0}84_{\pm 10.8} $ & $\phantom{-} \phantom{0}7_{\pm 7.1} $ & $\phantom{-} 11_{\pm 8.3} $ \\
    17 & llama-3-70b-instruct & $1202_{\pm 2.5} $ & $\phantom{-} 22_{\pm 4.1} $ & $-\phantom{0}32_{\pm 8.0} $ & $-\phantom{0}5_{\pm 5.3} $ & $\phantom{-} \phantom{0}0_{\pm 6.3} $ \\
    53 & mixtral-8x7b-instruct-v0.1 & $1114_{\pm 0.0} $ & $\phantom{-} \phantom{0}0_{\pm 0.0} $ & $\phantom{-} \phantom{00}0_{\pm 0.0} $ & $\phantom{-} \phantom{0}0_{\pm 0.0} $ & $\phantom{-} \phantom{0}0_{\pm 0.0} $ \\
    \bottomrule
    \end{tabular}
\end{table}

==> paper_files/impact.tex <==
\section*{Impact Statement}

Language models are applicable to a wide range of tasks. The use of univariate metrics to evaluate them is therefore not sufficient to capture the full complexity of these models and the tasks they need to solve. \tool acknowledges this by providing a way to evaluate models across multiple dimensions simultaneously and thus brings multidimensionality to the forefront of language model evaluation. Wide adoption of a multivariate approach will lead to a more nuanced understanding of language model capabilities, highlighting their strengths and weaknesses more effectively. Furthermore, \tool's ability to detect biases and dependencies can help the development of techniques to reduce the effect of these biases and improve the fairness of the evaluation.

==> paper_files/introduction.tex <==
\section{Introduction}
\vspace{-1mm}
Large language models (LLMs) have become powerful tools across a wide range of tasks, sometimes even outperforming human experts \citep{gpt4,claude,gemini,llama3modelcard}. To evaluate and compare the performance of LLMs, various benchmarks \citep{gsm8k,arc,mmlu} and evaluation frameworks \citep{eval-harness,helm} have been developed. These benchmarks aim to provide a comprehensive evaluation of LLM capabilities across tasks such as code completion, mathematical problem-solving, and multilingual understanding. However, the reliability of these benchmarks to accurately estimate model performance has been questioned due to various concerns about data contamination \citep{contaminationattacks,gsm1k}, errors in ground-truth solutions \citep{gema2024are}, and the discrepancy between benchmarks and real-world performance \citep{lin2024wildbench}.
\vspace{-1mm}
\paragraph{Ratings for LLMs} To evaluate LLMs more accurately in real-world scenarios, recent works have made use of rating-based evaluations with human or LLM-based judges \citep{chatbot_arena, lin2024wildbench,alpacelengthcontrolled}.
These ratings reflect the relative performance of LLMs on specific tasks and are used to construct leaderboards indicating their real-world performance. As shown in \cref{fig:overview}, ratings are derived from preference datasets containing samples consisting of a query $Q$, a response by two models $m^{(0)}$ and $m^{(1)}$, a judge $J$, and a judgment indicating the preferred response $r$. We illustrate human preference datasets for several tasks like code-based (\raisebox{-0.2\height}{\includegraphics[width=0.35cm]{figures/overview/code.png}}), mathematical (\raisebox{-0.2\height}{\includegraphics[width=0.35cm]{figures/overview/calculator.png}}), and Chinese (\raisebox{-0.2\height}{\includegraphics[width=0.35cm]{figures/overview/dragon.png}}) questions, along with a preference dataset using an LLM-based judge (\raisebox{-0.2\height}{\includegraphics[width=0.35cm]{figures/overview/bot.png}}).
Current methods fit each task separately using maximum likelihood estimation (MLE) to obtain ratings $R_{\text{task}}^i$ for each model $m_i$ that predict the judge's preferences as accurately as possible.
\vspace{-1mm}
\paragraph{Limitations of Current Rating Systems} However, current rating systems suffer from several critical limitations. First, it is widely recognized that judges are influenced by biases that significantly affect their preferences \citep{humanfeedback,wu2023style,shi2024judging,chen2024humans}. Yet, current rating systems are not expressive enough to capture these biases, leading to unfair comparisons of performance. Second, obtaining human annotations is very expensive. However, current systems are sample inefficient and do not take measures to reduce costs. This inefficiency makes it hard for resource-constrained LLM practitioners to use human evaluation for their tasks. Finally, the wide applicability of LLMs requires a comprehensive evaluation system to compare model performance across tasks. Yet, current rating systems suffer from shift-invariance, meaning that rating optimality is preserved when shifting all ratings by an arbitrary constant. For instance, all code-based ratings $R_{\includegraphics[width=0.22cm]{figures/overview/code.png}}^m$ can be shifted upwards by $40$ points while maintaining optimality, making the ratings on this task much higher than those on other tasks and rendering direct comparisons meaningless.

\begin{figure*}[t]
    \centering
    \resizebox{\linewidth}{!}{
        \input{figures/overview}
    }
    \vspace{-5mm}
    \caption[]{Overview of \tool. Given preference datasets of $n$ samples for $k$ models over various tasks, the standard approach needs to fit separate and independent ratings for each task and cannot leverage continuous features. In contrast, \tool fits a single linear model for all tasks and can leverage continuous features. Attribution in \cref{app:attribution}.}
    \label{fig:overview}
    \vspace{-2mm}
\end{figure*}

\paragraph{This Work: \tool} To address these limitations, we introduce \tool, an expressive rating system designed to model shared continuous features and biases influencing judge preferences. As illustrated in \cref{fig:overview}, \tool fits all preference datasets simultaneously using maximum a posteriori (MAP) estimation, i.e. using maximum likelihood estimation with additional priors on all parameters. These priors enable a more robust estimation of model ratings and act as a regularizer to prevent overfitting. Specifically, for each model $m$, a base rating $R^m_\text{base}$ is optimized to reflect overall performance across tasks. Task-specific modifiers $\beta^m_\text{task}$ are then added to this base rating to derive ratings for individual tasks. Additionally, shared parameters across all models $\alpha_\text{bias}$ capture the influence of features such as answer length (\raisebox{-0.2\height}{\includegraphics[width=0.35cm]{figures/overview/length.png}}) and readability (\raisebox{-0.2\height}{\includegraphics[width=0.35cm]{figures/overview/guideline.png}}) on preferences.


\paragraph{Benefits of \tool} 
\tool addresses previous limitations by design. By modeling shared features, \tool is the first rating system that can quantify biases affecting judge preferences by estimating their impact on model ratings. For instance, we find that answer length bias boosts ratings significantly by 41 points in the Chatbot Arena \citep{chatbot_arena}. Additionally, \tool improves sample efficiency and reduces the costs of evaluations for new tasks by up to $77\%$ when collecting $10000$ human annotations. \tool can also leverage LLM-based evaluations or traditional benchmarks to obtain ratings for human evaluation, allowing us to reduce its cost by respectively $38\%$ and $41\%$ when collecting $10000$ samples. Furthermore, \tool is not shift-invariant, enabling the construction of a leaderboard that offers detailed insights into each LLM's performance across different tasks, unlike previous approaches. Finally, we provide convergence guarantees and prove the optimality of \tool.

\paragraph{Main Contributions} In summary, our main contributions are:
\vspace{-2mm}
\begin{itemize}
    \setlength\itemsep{0.05em}
    \item Introducing \tool, a multivariate rating system based on MAP estimation (\cref{sec:tool}).
    \item Detecting the influence of several judge biases in human and LLM-based evaluations and for the first time estimating their effect on model ratings (\cref{sec:experiments:bias}).
    \item Demonstrating that \tool improves sample efficiency, reducing the cost of human evaluation by up to $77\%$ for new tasks and by $41\%$ for new models (\cref{sec:experiments:convergence}).
    \item Providing a multivariate leaderboard using \tool, enabling relative model performance comparisons across tasks (\cref{sec:experiments:leaderboards}).
\end{itemize}

==> paper_files/limitations.tex <==
\section{Limitations}\label{sec:limitations}

We briefly discuss the limitations of \tool. First, while \tool provides a way to measure model strengths and weaknesses, these comparisons are relative to the other models in the leaderboard and do not provide an absolute measure of model performance. For instance, if \emph{all} models in the leaderboard perform well on one task, and poorly on another, the leaderboard will not reflect this absolute weakness. Instead, it will only show weaknesses relative to the average performance of the models. This is a fundamental limitation of rating systems and cannot be solved by any system that works solely based on preference data. To obtain absolute measures of model performance additional data sources, such as traditional benchmarks, are required. 

Furthermore, \tool still requires significant manual inspection and tuning since users must determine the modeling parameters and functions that constitute the rating, a process that can be time-consuming. A more automatic discovery of interesting and relevant dimensions, especially for bias detection, would help mitigate this issue. 

==> paper_files/multi.tex <==
\section{\tool}\label{sec:tool}

We now introduce \tool, a multivariate rating system specifically designed for language model evaluation. This section first outlines the four design goals for an effective LLM rating system and then explains \tool and how it meets these objectives.

\subsection{Design Goals for LLM Rating System}

\paragraph{1) Quantify Biases} Both human and LLM-based judges are influenced by biases that affect their preferences \citep{humanfeedback,wu2023style,shi2024judging,chen2024humans}. A robust rating system must capture and quantify these biases to ensure fair comparisons of LLM performance, regardless of the judge. Current rating systems are predominantly univariate and are therefore unable to include the necessary extra parameters to capture these biases. Only AlpacaEval \citep{alpacelengthcontrolled} accounts for length bias, where the length of the model answer significantly influences the judge's preference. However, its fitted coefficient is not directly interpretable and does not quantify the bias's influence on ratings.
\vspace{-1mm}

\paragraph{2) Leverage Existing Information} Leveraging existing information can make a rating system more sample efficient and reduce evaluation costs. This information can come from LLM-based evaluations or traditional benchmarks, both of which indicate model performance and should therefore give valuable information that can improve sample efficiency. However, current rating systems start from scratch for each new task and model.

\vspace{-1mm}

\paragraph{3) Task Comparability} Univariate rating systems cannot directly compare ratings across tasks. This is due to shift-invariance, meaning that adding a constant $c \in \mathbb{R}$ to all ratings does not change their optimality. Specifically, the loss of ratings $\mathbf{R}$ on a dataset $D$ is invariant under the transformation $\mathbf{R} \rightarrow\mathbf{R} + c$, i.e. $\mathcal{L}(D, \mathbf{R}) = \mathcal{L}(D, \mathbf{R} + c)$. Therefore, if $\mathbf{R}_1$ and $\mathbf{R}_2$ are the optimal ratings for two different tasks, the rating difference for a specific model $R_1^m - R_2^m$ can be shifted by any constant $c$ without losing optimality. This makes it impossible to see how many rating points a model gained or lost from one task to another. A good rating system should eliminate this issue, allowing accurate performance comparisons of the same LLM across different tasks. 
\vspace{-1mm}

\paragraph{4) Optimality} Rating systems aim to predict the outcomes of games as accurately as possible. It can be shown that in the limit of infinite data, the univariate rating system presented in \cref{sec:background} obtains the highest possible accuracy. While infinite data is not practically achievable, any new rating system should retain this optimality.
\subsection{\tool}
\paragraph{Modeling Features} Features can be continuous, like the length of an answer, or discrete, like the task of the query. We model each feature as a function $f \colon G \times \{0,1\} \rightarrow \mathbb{R}$ that maps a game $g \in G$ and a boolean $i$ to a number quantifying the presence of this feature. The boolean $i$ specifies whether the model for which we want to compute the feature is the first or second model in the game.

\paragraph{Modeling Ratings} It is essential to model ratings as a function of these features to capture biases and measure task-specific ratings. For this purpose, we first note that ratings must be game-dependent to incorporate game-dependent features like query task or answer length. Furthermore, judge-specific biases are model-independent and must therefore be measured using parameters that are shared across all models. Finally, it is important that ratings remain interpretable and practical for leaderboards. Therefore, the rating for model $m$ in game $g$ is modeled using the linear model
\begin{equation}\label{eq:multi-bradley-terry}
R^{m}(g) = R^{m}_\text{base} + \sum_{j=1}^{d} \alpha_j f_j(g, \iverson{g_{m_1} = m})+ \sum_{j=1}^{d'} \beta^{m}_j f_j'(g, \iverson{g_{m_1} = m}).
\end{equation}
Here, $R^{m}_\text{base} \in \mathbb{R}$ is the base rating, $d$ and $d'$ are the number of features in the respective sums, $\alpha_j \in \mathbb{R}$ is the weight for feature $f_j$ and is shared across all models, $\beta^{m}_j \in \mathbb{R}$ is the model-specific weight for feature $f_j'$, and $\iverson{\dots}$ is the indicator function. Importantly, \cref{eq:multi-bradley-terry} serves as the key element of \tool that enables it to incorporate all design goals. Indeed, the shared parameters measure the biases in the judge's preferences, addressing the first design goal. To obtain task-specific ratings, we introduce a task-specific feature $f_\text{task}'(g, i) = \iverson{g \in D_{\text{task}}}$, where $D_{\text{task}}$ represents the set of all task-related queries. We then define the task-specific ratings as $R^{m}_{\text{task}} = R^{m}_\text{base} + \beta^{m}_\text{task}$. While this assumes no additional task-specific features are used, the definition can be easily extended to incorporate them, ensuring that ratings remain adaptable to varying evaluation contexts.

\paragraph{Optimization Objective} We perform MAP estimation with a normal prior on the weights $\alpha_j$ and $\beta^{m}_j$ with mean $0$ and deviations $\sigma_j$ and $\sigma'_j$ respectively. This leads to the optimization objective
\begin{equation}\label{eq:multi-logistic-loss}
    \mathcal{L}_\text{full}(D, \mathbf{R}_\text{base}, \boldsymbol{\alpha}, \boldsymbol{\beta}) = \sum_{g \in D} \mathcal{L}(\{g\}, R^1(g), \dots, R^k(g)) + \sum_{j=1}^{d} \frac{(\alpha_j)^2}{2 \left(\sigma_j\right)^2} +\sum_{m=1}^k\sum_{j=1}^{d'} \frac{(\beta^{m}_j)^2}{2 \left(\sigma_j'\right)^2},
\end{equation}
where $\mathbf{R}_\text{base}$ is the vector of base ratings, $\boldsymbol{\alpha}$ is the vector of shared weights, $\boldsymbol{\beta}$ is the matrix of model-specific weights, and ratings are computed using \cref{eq:multi-bradley-terry}. In contrast to the loss function presented in \cref{sec:background}, the dataset $D$ can contain games from different tasks.

Using MAP estimation instead of MLE allows \tool to incorporate information from existing tasks through its priors, thereby improving sample efficiency and reducing evaluation costs. Furthermore, evaluations with LLM-based judges can be considered as a distinct task and can therefore be used to improve sample efficiency. Traditional benchmarks can also be reinterpreted as preference datasets, where a question indicates a preference for models that answered correctly over those that did not. If the models are both (in)correct, the judge has no preference. We can therefore leverage all this information, ensuring that \tool satisfies the second design goal. 

However, while traditional benchmarks often predict a ranking similar to human preference data, their absolute performance measurements do not always align well with human ratings. For example, an easy benchmark will cluster all models close together because weaker models can answer most questions correctly, making it impossible for stronger models to achieve very high win rates against them. This makes \tool less effective, since the ratings from human preference data are spread further apart than those from these easy benchmarks. To address this issue, we introduce a hyperparameter that rescales the observed win rates of traditional benchmarks. This hyperparameter is optimized on the training data to realign \tool with the human preference data, allowing for a more effective combination of the two. Full details on this parameter are in \cref{app:details}.

Lastly, \tool removes shift-invariance. Indeed, task-specific ratings $R^m_\text{task} = R^{m}_\text{base} + \beta^{m}_\text{task}$ cannot be arbitrarily shifted compared to each other, since the priors on the task-specific weights $\boldsymbol{\beta}$ ensure that $\mathcal{L}_\text{full}(D, \mathbf{R}_\text{base}, \boldsymbol{\alpha}, \boldsymbol{\beta})\neq \mathcal{L}_\text{full}(D, \mathbf{R}_\text{base}, \boldsymbol{\alpha}, \boldsymbol{\beta} + c)$ for any non-zero constant $c$. This enables accurate comparisons of model performance across tasks and fulfills the third design goal.

\paragraph{Optimization} In \cref{app:proofs}, we show that the optimization objective from \cref{eq:multi-logistic-loss} is convex with  and twice differentiable with respect to $\mathbf{R}_\text{base}, \boldsymbol{\alpha}$ and $\boldsymbol{\beta}$, allowing us to use standard optimization techniques to optimize the loss with respect to these parameters. Specifically, we use Newton's method for the model-specific parameters and L-BFGS for the shared parameters. Furthermore, we prove in \cref{app:proofs} that, under weak assumptions, the obtained ratings converge to the ratings that maximize predictive capabilities and thus fulfill the final design goal.


\paragraph{Rating Uncertainty} We compute pivotal intervals using bootstrapping to obtain rating uncertainties \citep{bootstrapconfidence}. Specifically, given the actual estimate of the ratings $\hat{R}$ and $n$ bootstrap estimates $\hat{R}_1, \dots, \hat{R}_n$, the pivotal interval for a confidence $\alpha$ is $[\hat{R} - \hat{R}_{(1 - \alpha/2)}, \hat{R} - \hat{R}_{(\alpha/2)}]$, where $\hat{R}_{(1 - \alpha/2)}$ and $\hat{R}_{(\alpha/2)}$ are respectively the $1 - \alpha/2$ and $\alpha/2$ quantiles of the bootstrap estimates. For brevity, we report the $2\sigma$ confidence intervals obtained using bootstrapping in \cref{sec:experiments}, with detailed pivotal intervals reported in \cref{app:results}.

==> paper_files/related.tex <==
\section{Related Work}\label{sec:related}

\paragraph{Ratings} Rating systems have been used across various domains, such as sports \citep{elo2008rating,glicko,shelopugin2023ratings,eloplusplus,luis2012analysis}, gaming \citep{trueskill,trueskilltroughtime}, movies \citep{talatalinis2022ratingslib} and recommendation systems \citep{chen2018value,adomavicius2005incorporating,kong2019multidimensional}. The widely recognized Elo rating system \citep{elo2008rating} and its extensions such as Glicko \citep{glicko} are generic univariate systems based on the BT-model \citep{bradley1952rank} that are widely applicable. Furthermore, various rating systems have been developed for specific use cases and areas. For example, Elo++ \citep{eloplusplus} was specifically designed for chess, and TrueSkill \citep{trueskill,trueskilltroughtime} has been further developed specifically for multiplayer online games.

\paragraph{Ratings for LLMs} Preference datasets for LLMs have become common to evaluate model capabilities in areas lacking ground-truth benchmarks. The most popular one is the Chatbot Arena \citep{chatbot_arena}, which contains over one million user queries and evaluates models in various tasks such as code, math, and multilingual understanding. Wildbench \citep{lin2024wildbench}, MT-Bench \citep{zheng2023judging}, and AlpacaEval \citep{alpacelengthcontrolled} are LLM-based evaluation frameworks that have gained attention. Among these, AlpacaEval is the only one that applies a length-control bias  similar to \tool to obtain a higher correlation with human judges. However, this fitted bias is not directly interpretable and is less generic than the approach used in \tool. Additionally, \tool employs priors on various terms to improve sample efficiency and eliminate shift-invariance, which AlpacaEval lacks.

\paragraph{Multivariate Rating Systems} Multivariate rating systems have been used before in recommendation systems \citep{chen2018value,adomavicius2005incorporating,kong2019multidimensional}. These developed systems are extensions to the more classical Elo \citep{elo2008rating} and Glicko  \citep{glicko} rating systems. However, they are not directly applicable to LLM evaluation, as they do not take into account the specific biases and dependencies that are present in LLM evaluation. Furthermore, the limited numbers of models allow us to build an exact optimization algorithm, unlike in recommendation systems where approximate algorithms are necessary due to the high number of products.

\paragraph{Biases in Human and LLM-Based Evaluation} Several works have examined biases in both human and LLM-based evaluations \citep{humanfeedback,clark2021all,wang2023large,wu2023style,shi2024judging,chen2024humans,singhal2023long}. Typically, these studies introduce biases to model answers to observe their impact on judge preferences \citep{wu2023style,chen2024humans,singhal2023long,wang2023large}. Additionally, they also investigate bias by asking more specific questions to the judges, rather than simply asking their preference \citep{humanfeedback,wu2023style}. These techniques, however, do not apply to existing datasets and require additional annotations for specifically crafted answers. In contrast, \tool can be directly applied to existing datasets without further annotation.

